PDLogger: Automated Logging Framework for Practical Software Development

Logging is indispensable for maintaining the reliability and diagnosability of modern software, yet developers still struggle to decide where and how to log effectively. Existing automated logging techniques focus on isolated sub-tasks - predicting a single log position, level, or message - and therefore cannot produce complete, high-quality log statements that reflect real-world practice in which multiple logs often appear inside one method. They also neglect deeper semantic dependencies among methods and consider only a narrow set of candidate variables, leading to superficial or incomplete logs. In this paper, we present PDLogger, the first end-to-end log generation technique expressly designed for practical, multi-log scenarios. PDLogger operates in three phases. (1) Log position prediction: block-type-aware structured prompts guide a large language model (LLM) to suggest candidate positions across all control-flow blocks of a method. (2) Log generation: backward program slicing supplies precise inter-procedural control and data-dependency context, while an expanded variable extractor captures both member and external function expressions; the enriched prompt enables the LLM to emit a full log statement (position, level, message, variables). (3) Log refinement: level correction and context-sensitive deduplication prune false positives and redundant logs. We evaluate PDLogger on 3,113 log statements drawn from two widely used Java projects. Compared with the strongest prior systems, PDLogger improves log-position precision by 139.0 percent, F1 by 69.2 percent, level accuracy by 82.3 percent, variable precision by 131.8 percent, and message quality (BERTScore) by 65.7 percent. The framework consistently performs well with different mainstream LLMs, demonstrating robustness and generality. PDLogger's implementation is available as open source to foster future research and adoption.

==> abs.tex <==
%% article.
\begin{abstract}
%Logs, critical for system monitoring, troubleshooting, and auditing, are widely used in security analysis and business analytics, making them an indispensable component of modern software systems. Although multiple automated log generation techniques have been proposed, their practical adoption in software development remains challenging. State-of-the-art solutions lack sufficient contextual awareness and are designed to insert only one log statement in a method, significantly limiting their real-world applicability. Specifically, we identify three inherent limitations with existing schemes: lack of multi-log generation capability, insufficient semantic dependency context and limited logging variable scope. To this end, we propose \codename, the first high-accuracy log statement generation approach that is applicable to real-world development scenarios. First, \codename leverages static analysis to extract semantic dependency information, enabling the generation of more closely reflect the original intent of the ground truth and less redundant log statements. Second, it introduces a block-type-based structured prompting strategy to query the model in a more targeted manner, which significantly reduces the false positive rate of log position prediction in the multi-log prediction setting. Finally, performing function-aware extension by incorporating function information into the variable list. The evaluation results demonstrate that \codename outperforms the state-of-the-art approach by 139.00\% in log position precision, 69.20\% in F1 score, 82.30\% in logging level accuracy, 131.80\% in variable precision, and 65.70\% in BERTScore for log message generation. Furthermore, \codename consistently achieves strong performance across a variety of large language models, indicating its robust generalizability.
Logging is indispensable for maintaining the reliability and diagnosability of modern software, yet developers still struggle to decide where and how to log effectively. Existing automated logging techniques focus on isolated sub-tasks—predicting a single log position, level, or message—and therefore cannot produce complete, high-quality log statements that reflect real-world practice in which multiple logs often appear inside one method. They also neglect deeper semantic dependencies among methods and consider only a narrow set of candidate variables, leading to superficial or incomplete logs. In this paper, we present PDLogger, the first end-to-end log generation technique expressly designed for practical, multi-log scenarios. PDLogger operates in three phases. (1) Log position prediction: block-type–aware structured prompts guide a large language model (LLM) to suggest candidate positions across all control-flow blocks of a method. (2) Log generation: backward program slicing supplies precise inter-procedural control‐ and data-dependency context, while an expanded variable extractor captures both member and external function expressions; the enriched prompt enables the LLM to emit a full log statement (position, level, message, variables). (3) Log refinement: level correction and context-sensitive deduplication prune false positives and redundant logs. We evaluate PDLogger on 3,113 log statements drawn from two widely used Java projects. Compared with the strongest prior systems, PDLogger improves log-position precision by 139.0\%, F1 by 69.2\%, level accuracy by 82.3\%, variable precision by 131.8\%, and message quality (BERTScore) by 65.7\%. The framework consistently performs well with different mainstream LLMs, demonstrating robustness and generality. PDLogger’s implementation is available as open source to foster future research and adoption.
\end{abstract}



% \begin{CCSXML}
% <ccs2012>
%  <concept>
%   <concept_id>00000000.0000000.0000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>500</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>300</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
%  <concept>
%   <concept_id>00000000.00000000.00000000</concept_id>
%   <concept_desc>Do Not Use This Code, Generate the Correct Terms for Your Paper</concept_desc>
%   <concept_significance>100</concept_significance>
%  </concept>
% </ccs2012>
% \end{CCSXML}

% \ccsdesc[500]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[300]{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc{Do Not Use This Code~Generate the Correct Terms for Your Paper}
% \ccsdesc[100]{Do Not Use This Code~Generate the Correct Terms for Your Paper}

% %%
% %% Keywords. The author(s) should pick words that accurately describe
% %% the work being presented. Separate the keywords with commas.
% \keywords{logging, large language model, software maintenance}
% %% A "teaser" image appears between the author and affiliation
% %% information and the body of the document, and typically spans the
% %% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}
